FedNorm: Modality-Based Normalization in Federated Learning for Multi-Modal Liver Segmentation

Given the high incidence and effective treatment options for liver diseases, they are of great socioeconomic importance. One of the most common methods for analyzing CT and MRI images for diagnosis and follow-up treatment is liver segmentation. Recent advances in deep learning have demonstrated encouraging results for automatic liver segmentation. Despite this, their success depends primarily on the availability of an annotated database, which is often not available because of privacy concerns. Federated Learning has been recently proposed as a solution to alleviate these challenges by training a shared global model on distributed clients without access to their local databases. Nevertheless, Federated Learning does not perform well when it is trained on a high degree of heterogeneity of image data due to multi-modal imaging, such as CT and MRI, and multiple scanner types. To this end, we propose Fednorm and its extension \fednormp, two Federated Learning algorithms that use a modality-based normalization technique. Specifically, Fednorm normalizes the features on a client-level, while Fednorm+ employs the modality information of single slices in the feature normalization. Our methods were validated using 428 patients from six publicly available databases and compared to state-of-the-art Federated Learning algorithms and baseline models in heterogeneous settings (multi-institutional, multi-modal data). The experimental results demonstrate that our methods show an overall acceptable performance, achieve Dice per patient scores up to 0.961, consistently outperform locally trained models, and are on par or slightly better than centralized models.

==> algorithms/mode-normalization-testing.tex <==
% !TeX root = ../main.tex
% Add the above to each chapter to make compiling the PDF easier in some editors.
\begin{algorithm}[ht]
	\begin{algorithmic}[1]
		\FOR{$n = 1$ to $N$}
			\FOR{$m = 1$ to $M$}
				\STATE $g_{nm} \leftarrow \big[\sigma \circ \Psi(\boldsymbol{x}_n)\big]_m$\ \ \ // \emph{Compute mode assignments}
				\STATE $\boldsymbol{\mu}_m \leftarrow \overline{\langle \boldsymbol{x} \rangle}_m$\ \ \ // \emph{Estimate for mean}
				\STATE $\boldsymbol{\sigma}_m^2 \leftarrow \overline{\langle \boldsymbol{x}^2 \rangle}_m - \overline{\langle \boldsymbol{x} \rangle}_m^2$\ \ \ // \emph{Compute estimate for variance}
				\STATE $\boldsymbol{y}_{nm} \leftarrow g_{nm} (\boldsymbol{x}_n \ominus \boldsymbol{\mu}_m) \oslash \sqrt{\boldsymbol{\sigma}_m^2 + \boldsymbol{\varepsilon}}$\ \ \ // \emph{Normalize sample with estimates}
			\ENDFOR
		\ENDFOR
		\RETURN $\big\{\boldsymbol{\alpha} \odot \sum_{m=1}^M \boldsymbol{y}_{nm} \oplus \boldsymbol{\beta}\big\}_{n=1}^N$
	\end{algorithmic}
	\caption[Mode Normalization: Test Phase]{Mode Normalization: Test phase. $\boldsymbol{\varepsilon} = \varepsilon \cdot \boldsymbol{1}_C$ is a $C$-dimensional
											vector filled with a small positive value $\varepsilon$ for numerical stability. The running means
											$\overline{\langle \boldsymbol{x} \rangle}_m$ and $\overline{\langle \boldsymbol{x}^2 \rangle}_m$ are computed in the
											training phase (\Cref{alg:mode-normalization-training}). Algorithm adapted from
											\citeauthor{ModeNormalization}~\citep[Algorithm 2]{ModeNormalization}.}\label{alg:mode-normalization-testing}
\end{algorithm}

% Original algorithm from paper
% \begin{algorithm}[ht]
% 	\begin{algorithmic}
% 		\vspace*{.2cm}
% 		\STATE {\textbf{Input:}} refer to Alg.\ \ref{alg:mode-normalization-training}.
% 		\vspace*{.2cm}
% 		\STATE \hspace*{.23cm} Compute expert assignments:
% 		\vspace*{.2cm}
% 		% \STATE \hspace*{.6cm} $g_{nk} \leftarrow \text{softmax} \big[\Psi(x_n)\big]_k$
% 		\STATE \hspace*{.6cm} $g_{nk} \leftarrow \big[\sigma \circ \Psi(x_n)\big]_k$
% 		\vspace*{.2cm}
% 		\FOR{$n = 1$ to $N$}
% 		\vspace*{.2cm}
% 		\STATE Normalize samples with running average of component-wise estimators:
% 		\vspace*{.2cm}
% 		\STATE \hspace{.2cm} $\mu_k \leftarrow \overline{\langle x \rangle}_k$
% 		\STATE \hspace{.2cm} $\sigma_k^2 \leftarrow \overline{\langle x^2 \rangle}_k - \overline{\langle x \rangle}_k^2$
% 		\STATE \hspace{.2cm} $y_{nk} \leftarrow g_{nk} \frac{x_n - \mu_k}{\sqrt{\sigma_k^2 + \varepsilon}} $
% 		\vspace*{.2cm}
% 		\ENDFOR
% 		% \vspace*{.1cm}
% 		\STATE {\bfseries Return:} $\{\alpha \sum_k y_{nk} + \beta\}_{n=1,\dots,N}$
% 	\end{algorithmic}
% 	\caption[Mode Normalization: Test Phase]{Mode Normalization: Test phase.}\label{alg:mode-normalization-testing}
% \end{algorithm}

==> algorithms/mode-normalization-training.tex <==
% !TeX root = ../main.tex
% Add the above to each chapter to make compiling the PDF easier in some editors.
\begin{algorithm}[ht]
	\begin{algorithmic}[1]
		\FOR{$n = 1$ to $N$}
			\FOR{$m = 1$ to $M$}
				\STATE $g_{nm} \leftarrow \big[\sigma \circ \Psi(\boldsymbol{x}_n)\big]_m$\ \ \ // \emph{Compute mode assignments}
			\ENDFOR
		\ENDFOR
		\FOR{$m = 1$ to $M$}
			\STATE $\overline{\langle \boldsymbol{x} \rangle}_m \leftarrow \boldsymbol{0}_C$
			\STATE $\overline{\langle \boldsymbol{x}^2 \rangle}_m \leftarrow \boldsymbol{0}_C$
		\ENDFOR
		\FOR{$m = 1$ to $M$}
			\STATE // \emph{Determine new component-wise statistics:}
			\STATE $N_m \leftarrow \sum_{n=1}^N g_{nm}$
			\STATE $\langle \boldsymbol{x} \rangle_m \leftarrow \frac{1}{N_m} \sum_{n=1}^N g_{nm} \varphi(\boldsymbol{x}_n)$
			\STATE $\langle \boldsymbol{x}^2 \rangle_m \leftarrow \frac{1}{N_m} \sum_{n=1}^N g_{nm} \varphi(\boldsymbol{x}_n)^2$
			\STATE // \emph{Update running means:}
			\STATE $\overline{\langle \boldsymbol{x} \rangle}_m \leftarrow \lambda \langle \boldsymbol{x} \rangle_m + (1 - \lambda) \overline{\langle \boldsymbol{x} \rangle}_m$
			\STATE $\overline{\langle \boldsymbol{x}^2 \rangle}_m \leftarrow \lambda \langle \boldsymbol{x}^2 \rangle_m + (1 - \lambda) \overline{\langle \boldsymbol{x}^2 \rangle}_m$
		\ENDFOR
		\FOR{$n = 1$ to $N$}
			\FOR{$m = 1$ to $M$}
				\STATE $\boldsymbol{\mu}_m \leftarrow \langle \boldsymbol{x} \rangle_m$\ \ \ // \emph{Estimate for mean}
				\STATE $\boldsymbol{\sigma}_m^2 \leftarrow \langle \boldsymbol{x}^2 \rangle_m - \langle \boldsymbol{x} \rangle_m^2$\ \ \ // \emph{Compute estimate for variance}
				\STATE $\boldsymbol{y}_{nm} \leftarrow g_{nm} (\boldsymbol{x}_n \ominus \boldsymbol{\mu}_m) \oslash \sqrt{\boldsymbol{\sigma}_m^2 + \boldsymbol{\varepsilon}}$\ \ \ // \emph{Normalize sample with estimates}
			\ENDFOR
		\ENDFOR
		\RETURN $\big\{\boldsymbol{\alpha} \odot \sum_{m=1}^M \boldsymbol{y}_{nm} \oplus \boldsymbol{\beta}\big\}_{n=1}^N$
	\end{algorithmic}
	\caption[Mode Normalization: Training Phase]{Mode Normalization: Training phase. $\boldsymbol{\varepsilon} = \varepsilon \cdot \boldsymbol{1}_C$ is a
												$C$-dimensional vector filled with a small positive value $\varepsilon$ for numerical stability,
												$\boldsymbol{0}_C$ is the $C$-dimensional zero vector, and $\varphi: \mathbb{R}^{C \times H \times W} \to \mathbb{R}^C$
												is a function that takes the channel-wise mean over the height and width dimensions of its input.
												Algorithm adapted from \citeauthor{ModeNormalization}~\citep[Algorithm 1]{ModeNormalization} and their publicly available implementation~\citep{ModeNormalizationCode}.}\label{alg:mode-normalization-training}
\end{algorithm}

% Original algorithm from paper
% \begin{algorithm}[ht]
% 	\begin{algorithmic}
% 		\vspace*{.2cm}
% 		\STATE {\textbf{Input:}} parameters $\lambda, K$, batch of samples $\{x_n\}$, small $\varepsilon$, learnable $\alpha, \beta,\Psi \colon \mathcal X\to\mathbb R^K$.
% 		\vspace*{.2cm}
% 		\STATE \hspace*{.23cm} Compute expert assignments:
% 		\vspace*{.2cm}
% 		% \STATE \hspace*{.6cm} $g_{nk} \leftarrow \text{softmax} \big[\Psi(x_n)\big]_k$
% 		\STATE \hspace*{.6cm} $g_{nk} \leftarrow \big[\sigma \circ \Psi(x_n)\big]_k$
% 		\vspace*{.2cm}
% 		\FOR{$k = 1$ to $K$}
% 		\vspace*{.2cm}
% 		\STATE Determine new component-wise statistics:
% 		\vspace*{.2cm}
% 		\STATE \hspace{.2cm} $N_{k} \leftarrow \sum_n g_{nk}$
% 		\STATE \hspace{.2cm} $\langle x \rangle_k \leftarrow \frac{1}{N_k} \sum_{n} g_{nk} x_n$
% 		\STATE \hspace{.2cm} $\langle x^2 \rangle_k \leftarrow \frac{1}{N_k} \sum_{n} g_{nk} x^2_n$
% 		\vspace*{.2cm}
% 		\STATE Update running means:
% 		\vspace*{.2cm}
% 		\STATE \hspace{.2cm} $\overline{\langle x \rangle}_k \leftarrow \lambda \langle x \rangle_k + (1 - \lambda) \overline{\langle x \rangle}_k $
% 		\STATE \hspace{.2cm} $\overline{\langle x^2 \rangle}_k \leftarrow \lambda \langle x^2 \rangle_k   + (1 - \lambda) \overline{\langle x^2 \rangle}_k $
% 		\vspace*{.2cm}
% 		\ENDFOR
% 		% \vspace*{.2cm}
% 		\FOR{$n = 1$ to $N$}
% 		\vspace*{.2cm}
% 		\STATE Normalize samples with component-wise estimators:
% 		\vspace*{.2cm}
% 		\STATE \hspace{.2cm} $\mu_k \leftarrow \langle x \rangle_k$
% 		\vspace*{.12cm}
% 		\STATE \hspace{.2cm} $\sigma_k^2 \leftarrow \langle x^2 \rangle_k - \langle x \rangle_k^2$
% 		% \STATE \hspace{.2cm} $y_{nk} \leftarrow g_{nk} \big[ \alpha_k \frac{x_n - \mu_k}{\sqrt{\sigma_k^2 + \varepsilon}} + \beta_k \big]$
% 		\STATE \hspace{.2cm} $y_{nk} \leftarrow g_{nk} \frac{x_n - \mu_k}{\sqrt{\sigma_k^2 + \varepsilon}} $
% 		\ENDFOR
% 		% \vspace*{.1cm}
% 		\STATE {\bfseries Return:} $\{\alpha \sum_k y_{nk} + \beta\}_{n=1,\dots,N}$
% 	\end{algorithmic}
% 	\caption[Mode Normalization: Training Phase]{Mode Normalization: Training phase.}\label{alg:mode-normalization-training}
% \end{algorithm}

==> tables/client-refinement-non-iid-3-old.tex <==
% !TeX root = ../main.tex
% Add the above to each chapter to make compiling the PDF easier in some editors.
\begin{table*}[ht]
	\caption[Local Client Refinement: Non-IID 3 Setting]{Local client refinement for federated models in the Non-IID 3 setting on the test set of each client. The local models and the centralized model are not refined. The relative improvement based on \Cref{eqn:relative-improvement} is given for the score after refinement over the score before refinement.}\label{tab:comparison-non-iid-3}
	\centering
	\begin{adjustbox}{max width=\textwidth, max height=0.45\textheight}
		\begin{tabular}{c c c c c c}
			\toprule
			\multirow{2}{*}{\textbf{Client}}									& \multirow{2}{*}{\textbf{Modality}}	& \multirow{2}{*}{\textbf{Methods}}	& \textbf{Dice per Patient} $\boldsymbol{\uparrow}$	& \textbf{Dice per Patient} $\boldsymbol{\uparrow}$	& \textbf{Relative}			\\
																				&										&										& \textbf{(Before Refinement)}						& \textbf{(After Refinement)}						& \textbf{Improvement (\%)}	\\
			\midrule
			\multirow{8}{*}{Multi-Atlas}										& \multirow{8}{*}{CT}					& Local									& $0.867\,(0.889) \pm 0.061$						& $0.867\,(0.889) \pm 0.061$ 						& -							\\
																				  \cdashline{3-6}
																				&										& FedAvg								& $0.924\,(0.934) \pm 0.027$						& $0.945\,(0.947) \pm 0.017$ 						& 2.273						\\
																				&										& FedVC									& $0.886\,(0.892) \pm 0.048$						& $0.906\,(0.912) \pm 0.028$ 						& 2.257						\\
																				&										& SiloBN								& $0.889\,(0.896) \pm 0.051$						& $0.938\,(0.944) \pm 0.022$ 						& 5.512						\\
																				&										& FedBN									& $0.899\,(0.932) \pm 0.073$						& $0.945\,(0.952) \pm 0.020$ 						& 5.117						\\
																				&										& FedNorm+								& $0.931\,(0.939) \pm 0.025$						& $0.942\,(0.950) \pm 0.023$ 						& 1.182						\\
																				  \cdashline{3-6}
																				&										& Centralized							& $0.927\,(0.941) \pm 0.030$						& $0.927\,(0.941) \pm 0.030$ 						& -							\\
			\midrule
			\multirow{8}{*}{3D-IRCADb}											& \multirow{8}{*}{CT}					& Local									& $0.908\,(0.914) \pm 0.026$						& $0.908\,(0.914) \pm 0.026$						& -							\\
																				  \cdashline{3-6}
																				&										& FedAvg								& $0.926\,(0.942) \pm 0.040$						& $0.951\,(0.956) \pm 0.018$ 						& 2.7						\\
																				&										& FedVC									& $0.915\,(0.928) \pm 0.039$						& $0.919\,(0.923) \pm 0.034$ 						& 0.437						\\
																				&										& SiloBN								& $0.948\,(0.958) \pm 0.027$						& $0.952\,(0.959) \pm 0.026$ 						& 0.422						\\
																				&										& FedBN									& $0.941\,(0.953) \pm 0.031$						& $0.954\,(0.961) \pm 0.019$ 						& 1.382						\\
																				&										& FedNorm+								& $0.948\,(0.949) \pm 0.016$						& $0.959\,(0.966) \pm 0.016$ 						& 1.16						\\
																				  \cdashline{3-6}
																				&										& Centralized							& $0.956\,(0.960) \pm 0.015$						& $0.956\,(0.960) \pm 0.015$ 						& -							\\
			\midrule
			\multirow{8}{*}{\shortstack{CHAOS19 MR\\T1 Water}}					& \multirow{8}{*}{MRI}					& Local									& $0.646\,(0.760) \pm 0.266$						& $0.646\,(0.760) \pm 0.266$ 						& -	 						\\
																				  \cdashline{3-6}
																				&										& FedAvg								& $0.468\,(0.512) \pm 0.334$						& $0.783\,(0.819) \pm 0.096$ 						& 67.308					\\
																				&										& FedVC									& $0.314\,(0.242) \pm 0.323$						& $0.741\,(0.756) \pm 0.054$ 						& 135.987					\\
																				&										& SiloBN								& $0.609\,(0.652) \pm 0.223$						& $0.815\,(0.870) \pm 0.128$ 						& 33.826					\\
																				&										& FedBN									& $0.563\,(0.631) \pm 0.332$						& $0.877\,(0.906) \pm 0.061$ 						& 55.773					\\
																				&										& FedNorm+								& $0.779\,(0.805) \pm 0.094$						& $0.825\,(0.854) \pm 0.150$ 						& 5.905						\\
																				  \cdashline{3-6}
																				&										& Centralized							& $0.826\,(0.873) \pm 0.090$						& $0.826\,(0.873) \pm 0.090$ 						& -							\\
			\midrule
			\multirow{8}{*}{\shortstack{KORA\\T1 Water (1)}}					& \multirow{8}{*}{MRI}					& Local									& $0.864\,(0.859) \pm 0.054$						& $0.864\,(0.859) \pm 0.054$ 						& -	 						\\
																				  \cdashline{3-6}
																				&										& FedAvg								& $0.924\,(0.936) \pm 0.034$						& $0.929\,(0.939) \pm 0.034$ 						& 0.541						\\
																				&										& FedVC									& $0.920\,(0.914) \pm 0.025$						& $0.899\,(0.910) \pm 0.043$ 						& -2.283					\\
																				&										& SiloBN								& $0.934\,(0.944) \pm 0.029$						& $0.930\,(0.938) \pm 0.027$ 						& -0.428					\\
																				&										& FedBN									& $0.936\,(0.946) \pm 0.029$						& $0.932\,(0.939) \pm 0.024$						& -0.427					\\
																				&										& FedNorm+								& $0.938\,(0.945) \pm 0.025$						& $0.928\,(0.937) \pm 0.031$ 						& -1.066					\\
																				  \cdashline{3-6}
																				&										& Centralized							& $0.936\,(0.944) \pm 0.025$						& $0.936\,(0.944) \pm 0.025$ 						& -							\\
			\midrule
			\multirow{8}{*}{\shortstack{SLIVER07\\+ KORA T1\\Water (2)}}		& \multirow{8}{*}{CT + MRI}				& Local									& $0.726\,(0.900) \pm 0.352$						& $0.726\,(0.900) \pm 0.352$ 						& -	 						\\
																				  \cdashline{3-6}
																				&										& FedAvg								& $0.742\,(0.922) \pm 0.367$						& $0.754\,(0.930) \pm 0.362$ 						& 1.617						\\
																				&										& FedVC									& $0.740\,(0.925) \pm 0.350$						& $0.739\,(0.909) \pm 0.347$ 						& -0.135					\\
																				&										& SiloBN								& $0.746\,(0.908) \pm 0.344$						& $0.768\,(0.930) \pm 0.341$ 						& 2.949						\\
																				&										& FedBN									& $0.745\,(0.933) \pm 0.369$						& $0.755\,(0.932) \pm 0.362$ 						& 1.342						\\
																				&										& FedNorm+								& $0.752\,(0.946) \pm 0.360$						& $0.756\,(0.923) \pm 0.364$ 						& 0.532						\\
																				  \cdashline{3-6}
																				&										& Centralized							& $0.848\,(0.940) \pm 0.174$						& $0.848\,(0.940) \pm 0.174$ 						& -							\\
			\midrule
			\multirow{8}{*}{\shortstack{LiTS17\\Site 2\\+ KORA T1\\Water (3)}}	& \multirow{8}{*}{CT + MRI}				& Local									& $0.879\,(0.917) \pm 0.093$						& $0.879\,(0.917) \pm 0.093$ 						& -	 						\\
																				  \cdashline{3-6}
																				&										& FedAvg								& $0.920\,(0.952) \pm 0.083$						& $0.910\,(0.949) \pm 0.095$ 						& -1.087					\\
																				&										& FedVC									& $0.901\,(0.929) \pm 0.089$						& $0.906\,(0.938) \pm 0.071$ 						& 0.555						\\
																				&										& SiloBN								& $0.937\,(0.953) \pm 0.039$						& $0.931\,(0.955) \pm 0.052$ 						& -0.64						\\
																				&										& FedBN									& $0.935\,(0.952) \pm 0.048$						& $0.926\,(0.946) \pm 0.055$						& -0.963					\\
																				&										& FedNorm+								& $0.947\,(0.952) \pm 0.023$						& $0.928\,(0.947) \pm 0.051$ 						& -2.006					\\
																				  \cdashline{3-6}
																				&										& Centralized							& $0.944\,(0.954) \pm 0.023$						& $0.944\,(0.954) \pm 0.023$ 						& -							\\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
\end{table*}

==> tables/client-refinement-non-iid-3.tex <==
% !TeX root = ../main.tex
% Add the above to each chapter to make compiling the PDF easier in some editors.
\begin{table*}[ht]
	\caption[Local Client Refinement: Non-IID 3 Setting]{Local client refinement on Non-IID 3 setting. Each global model (before refinement), which was computed by the
														corresponding algorithm during training, is refined on the training set of each client for $E = 1$ local
														epoch (after refinement). Local and centralized models are not refined. Performances are given with mean
														(median) and standard deviation Dice per patient. The last column gives the RI of the mean
														performance after refinement over the mean performance before refinement according to \Cref{eqn:relative-improvement}.
														A star ($^\ast$) before/behind a model name indicates that the results before/after refinement are
														statistically significant compared to the local model performance with a $p$-value $\leq 0.05$ using the unpaired two-sided t-test.
														The best model performance among the FL algorithms per client for each column is highlighted in bold. \fedavgm and \fednorm are not included in this table because \fedavgm
														fails during training in this setting and \fednorm cannot handle mixed-modality clients.}\label{tab:client-refinement-non-iid-3}
	\centering
	\begin{adjustbox}{max width=\textwidth, max height=0.45\textheight}
		\begin{tabular}{c c c c c}
			\toprule
			\multirow{2}{*}{\shortstack{\textbf{Client}\\\textbf{(Modality)}}}				& \multirow{2}{*}{\textbf{Algorithms}}	& \textbf{Dice per Patient} $\boldsymbol{\uparrow}$	& \textbf{Dice per Patient} $\boldsymbol{\uparrow}$	& \multirow{2}{*}{\textbf{RI [\%]} $\boldsymbol{\uparrow}$}	\\
																							&										& \textbf{(Before Refinement)}						& \textbf{(After Refinement)}						& 															\\
			\midrule
			\multirow{8}{*}{\shortstack{Multi-Atlas\\(CT)}}									& Local									& $0.867\,(0.889) \pm 0.061$						& $0.867\,(0.889) \pm 0.061$ 						& -															\\
																							 \cdashline{2-5}
																							& $^\ast$FedAvg$^\ast$~\cite{FedAvg}	& $0.924\,(0.934) \pm 0.027$						& $0.945\,(0.947) \pm 0.017$ 						& 2.273														\\
																							& FedVC$^\ast$~\cite{FedVC}			& $0.886\,(0.892) \pm 0.048$						& $0.906\,(0.912) \pm 0.028$ 						& 2.257														\\
																							& SiloBN$^\ast$~\cite{SiloBN}			& $0.889\,(0.896) \pm 0.051$						& $0.938\,(0.944) \pm 0.022$ 						& \textbf{5.512}											\\
																							& FedBN$^\ast$~\cite{FedBN}			& $0.899\,(0.932) \pm 0.073$						& $\boldsymbol{0.945\,(0.952) \pm 0.020}$ 			& 5.117														\\
																							& $^\ast$FedNorm+$^\ast$				& $\boldsymbol{0.931\,(0.939) \pm 0.025}$			& $0.942\,(0.950) \pm 0.023$ 						& 1.182														\\
																							 \cdashline{2-5}
																							& $^\ast$Centralized$^\ast$				& $0.927\,(0.941) \pm 0.030$						& $0.927\,(0.941) \pm 0.030$ 						& -															\\
			\midrule
			\multirow{8}{*}{\shortstack{3D-IRCADb\\(CT)}}									& Local									& $0.908\,(0.914) \pm 0.026$						& $0.908\,(0.914) \pm 0.026$						& -															\\
																							 \cdashline{2-5}
																							& FedAvg$^\ast$~\cite{FedAvg}			& $0.926\,(0.942) \pm 0.040$						& $0.951\,(0.956) \pm 0.018$ 						& \textbf{2.7}												\\
																							& FedVC~\cite{FedVC}					& $0.915\,(0.928) \pm 0.039$						& $0.919\,(0.923) \pm 0.034$ 						& 0.437														\\
																							& $^\ast$SiloBN$^\ast$~\cite{SiloBN}	& $\boldsymbol{0.948\,(0.958) \pm 0.027}$			& $0.952\,(0.959) \pm 0.026$ 						& 0.422														\\
																							& $^\ast$FedBN$^\ast$~\cite{FedBN}		& $0.941\,(0.953) \pm 0.031$						& $0.954\,(0.961) \pm 0.019$ 						& 1.382														\\
																							& $^\ast$FedNorm+$^\ast$				& $\boldsymbol{0.948\,(0.949) \pm 0.016}$			& $\boldsymbol{0.959\,(0.966) \pm 0.016}$ 			& 1.16														\\
																							 \cdashline{2-5}
																							& $^\ast$Centralized$^\ast$				& $0.956\,(0.960) \pm 0.015$						& $0.956\,(0.960) \pm 0.015$ 						& -															\\
			\midrule
			\multirow{8}{*}{\shortstack{CHAOS19 MR\\T1 Water\\(MRI)}}						& Local									& $0.646\,(0.760) \pm 0.266$						& $0.646\,(0.760) \pm 0.266$ 						& -	 														\\
																							 \cdashline{2-5}
																							& FedAvg~\cite{FedAvg}					& $0.468\,(0.512) \pm 0.334$						& $0.783\,(0.819) \pm 0.096$ 						& 67.308													\\
																							& $^\ast$FedVC~\cite{FedVC}			& $0.314\,(0.242) \pm 0.323$						& $0.741\,(0.756) \pm 0.054$ 						& \textbf{135.987}											\\
																							& SiloBN~\cite{SiloBN}					& $0.609\,(0.652) \pm 0.223$						& $0.815\,(0.870) \pm 0.128$ 						& 33.826													\\
																							& FedBN$^\ast$~\cite{FedBN}			& $0.563\,(0.631) \pm 0.332$						& $\boldsymbol{0.877\,(0.906) \pm 0.061}$ 			& 55.773													\\
																							& FedNorm+								& $\boldsymbol{0.779\,(0.805) \pm 0.094}$			& $0.825\,(0.854) \pm 0.150$ 						& 5.905														\\
																							 \cdashline{2-5}
																							& Centralized							& $0.826\,(0.873) \pm 0.090$						& $0.826\,(0.873) \pm 0.090$ 						& -															\\
			\midrule
			\multirow{8}{*}{\shortstack{KORA\\T1 Water (1)\\(MRI)}}							& Local									& $0.864\,(0.859) \pm 0.054$						& $0.864\,(0.859) \pm 0.054$ 						& -	 														\\
																							 \cdashline{2-5}
																							& $^\ast$FedAvg$^\ast$~\cite{FedAvg}	& $0.924\,(0.936) \pm 0.034$						& $0.929\,(0.939) \pm 0.034$ 						& \textbf{0.541}											\\
																							& $^\ast$FedVC~\cite{FedVC}			& $0.920\,(0.914) \pm 0.025$						& $0.899\,(0.910) \pm 0.043$ 						& -2.283													\\
																							& $^\ast$SiloBN$^\ast$~\cite{SiloBN}	& $0.934\,(0.944) \pm 0.029$						& $0.930\,(0.938) \pm 0.027$ 						& -0.428													\\
																							& $^\ast$FedBN$^\ast$~\cite{FedBN}		& $0.936\,(0.946) \pm 0.029$						& $\boldsymbol{0.932\,(0.939) \pm 0.024}$			& -0.427													\\
																							& $^\ast$FedNorm+$^\ast$				& $\boldsymbol{0.938\,(0.945) \pm 0.025}$			& $0.928\,(0.937) \pm 0.031$ 						& -1.066													\\
																							 \cdashline{2-5}
																							& $^\ast$Centralized$^\ast$				& $0.936\,(0.944) \pm 0.025$						& $0.936\,(0.944) \pm 0.025$ 						& -															\\
			\midrule
			\multirow{8}{*}{\shortstack{SLIVER07\\+ KORA T1\\Water (2)\\(CT + MRI)}}		& Local									& $0.726\,(0.900) \pm 0.352$						& $0.726\,(0.900) \pm 0.352$ 						& -	 														\\
																							 \cdashline{2-5}
																							& FedAvg~\cite{FedAvg}					& $0.742\,(0.922) \pm 0.367$						& $0.754\,(0.930) \pm 0.362$ 						& 1.617														\\
																							& FedVC~\cite{FedVC}					& $0.740\,(0.925) \pm 0.350$						& $0.739\,(0.909) \pm 0.347$ 						& -0.135													\\
																							& SiloBN~\cite{SiloBN}					& $0.746\,(0.908) \pm 0.344$						& $\boldsymbol{0.768\,(0.930) \pm 0.341}$ 			& \textbf{2.949}											\\
																							& FedBN~\cite{FedBN}					& $0.745\,(0.933) \pm 0.369$						& $0.755\,(0.932) \pm 0.362$ 						& 1.342														\\
																							& FedNorm+								& $\boldsymbol{0.752\,(0.946) \pm 0.360}$			& $0.756\,(0.923) \pm 0.364$ 						& 0.532														\\
																							 \cdashline{2-5}
																							& Centralized							& $0.848\,(0.940) \pm 0.174$						& $0.848\,(0.940) \pm 0.174$ 						& -															\\
			\midrule
			\multirow{8}{*}{\shortstack{LiTS17\\Site 2\\+ KORA T1\\Water (3)\\(CT + MRI)}}	& Local									& $0.879\,(0.917) \pm 0.093$						& $0.879\,(0.917) \pm 0.093$ 						& -	 														\\
																							 \cdashline{2-5}
																							& FedAvg~\cite{FedAvg}					& $0.920\,(0.952) \pm 0.083$						& $0.910\,(0.949) \pm 0.095$ 						& -1.087													\\
																							& FedVC~\cite{FedVC}					& $0.901\,(0.929) \pm 0.089$						& $0.906\,(0.938) \pm 0.071$ 						& \textbf{0.555}											\\
																							& $^\ast$SiloBN~\cite{SiloBN}			& $0.937\,(0.953) \pm 0.039$						& $\boldsymbol{0.931\,(0.955) \pm 0.052}$ 			& -0.64														\\
																							& FedBN~\cite{FedBN}					& $0.935\,(0.952) \pm 0.048$						& $0.926\,(0.946) \pm 0.055$						& -0.963													\\
																							& $^\ast$FedNorm+						& $\boldsymbol{0.947\,(0.952) \pm 0.023}$			& $0.928\,(0.947) \pm 0.051$ 						& -2.006													\\
																							 \cdashline{2-5}
																							& $^\ast$Centralized$^\ast$				& $0.944\,(0.954) \pm 0.023$						& $0.944\,(0.954) \pm 0.023$ 						& -															\\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
\end{table*}

==> tables/comparison-non-iid-1-2.tex <==
% !TeX root = ../main.tex
% Add the above to each chapter to make compiling the PDF easier in some editors.
\begin{table*}[ht]
	\caption[Comparison: Non-IID 1 and Non-IID 2 Settings]{Comparison on the Non-IID 1 and Non-IID 2 settings. The numbers give the performances of the local models, the centralized model, and the
															federated global models (without refinement at the clients) on the test set of each client. The performances are reported with Dice per
															patient and are given by mean (median) and standard deviation. Additionally, the RI according to \Cref{eqn:relative-improvement} is computed
															for the mean Dice per patient of the models from the FL algorithms and the centralized model over the local model
															performance. Hence, the RI is not reported for the local models. The best score from the federated models per client is highlighted
															in bold. A star ($^\ast$) before/behind (Non-IID 1/2 setting) the model name indicates that the results are statistically significant
															with a $p$-value $\leq 0.05$ using the unpaired two-sided t-test on the Dice per patient scores from the local model
															and the respective federated/centralized model.}\label{tab:comparison-non-iid-1-2}
	\centering
	\begin{adjustbox}{max width=\textwidth, max height=0.44\textheight}
		\begin{tabular}{c c c c c c}
			\toprule
			\multirow{2}{*}{\shortstack{\textbf{Client}\\\textbf{(Modality)}}}& \multirow{2}{*}{\textbf{Algorithms}}& \textbf{Non-IID 1}								& \textbf{RI (Non-IID 1)}								& \textbf{Non-IID 2}										& \textbf{RI (Non-IID 2)}									\\
																			&										& \textbf{Dice per Patient} $\boldsymbol{\uparrow}$	& \textbf{[\%]} $\boldsymbol{\uparrow}$					& \textbf{Dice per Patient} $\boldsymbol{\uparrow}$			& \textbf{[\%]} $\boldsymbol{\uparrow}$						\\
			\midrule
			\multirow{8}{*}{\shortstack{Multi-Atlas\\(CT)}}					& Local									& $0.867\,(0.889) \pm 0.061$						& -														& $0.867\,(0.889) \pm 0.061$								& -															\\
																			  \cdashline{3-6}
																			& FedAvg$^\ast$							& $0.871\,(0.878) \pm 0.072$						& 0.461													& $0.904\,(0.910) \pm 0.045$								& 4.268														\\
																			& $^\ast$FedAvgM$^\ast$					& $0.724\,(0.741) \pm 0.090$						& -16.494												& $0.574\,(0.584) \pm 0.164$								& -33.795													\\
																			& $^\ast$FedVC$^\ast$					& $0.826\,(0.822) \pm 0.046$						& -4.729												& $0.488\,(0.472) \pm 0.144$								& -43.714													\\
																			& $^\ast$SiloBN							& $0.932\,(0.943) \pm 0.028$						& 7.497													& $0.825\,(0.853) \pm 0.077$								& -4.844													\\
																			& $^\ast$FedBN$^\ast$					& $\boldsymbol{0.934\,(0.945) \pm 0.026}$			& $\boldsymbol{7.728}$									& $0.915\,(0.937) \pm 0.040$								& 5.536														\\
																			& $^\ast$FedNorm$^\ast$					& $0.905\,(0.929) \pm 0.049$						& 4.383													& $\boldsymbol{0.923\,(0.931) \pm 0.027}$					& $\boldsymbol{6.459}$										\\
																			& FedNorm+								& $0.871\,(0.878) \pm 0.074$						& 0.461													& $0.831\,(0.861) \pm 0.088$								& -4.152													\\
																			  \cdashline{3-6}
																			& $^\ast$Centralized$^\ast$				& $0.933\,(0.944) \pm 0.030$						& 7.612													& $0.937\,(0.947) \pm 0.024$								& 8.074														\\
			\midrule
			\multirow{8}{*}{\shortstack{3D-IRCADb\\(CT)}}					& Local									& $0.908\,(0.914) \pm 0.026$						& -														& $0.908\,(0.914) \pm 0.026$								& -															\\
																			  \cdashline{3-6}
																			& FedAvg$^\ast$							& $0.925\,(0.934) \pm 0.027$						& 1.872													& $0.942\,(0.942) \pm 0.022$								& 3.744														\\
																			& $^\ast$FedAvgM						& $0.323\,(0.240) \pm 0.238$						& -64.427												& $0.852\,(0.881) \pm 0.072$								& -6.167													\\
																			& FedVC$^\ast$							& $0.888\,(0.899) \pm 0.030$						& -2.203												& $0.817\,(0.841) \pm 0.051$								& -10.022													\\
																			& $^\ast$SiloBN$^\ast$					& $0.950\,(0.953) \pm 0.015$						& 4.626													& $0.950\,(0.952) \pm 0.017$								& 4.626														\\
																			& $^\ast$FedBN$^\ast$					& $\boldsymbol{0.955\,(0.951) \pm 0.016}$			& $\boldsymbol{5.176}$									& $\boldsymbol{0.960\,(0.959) \pm 0.012}$					& $\boldsymbol{5.727}$										\\
																			& $^\ast$FedNorm$^\ast$					& $0.942\,(0.948) \pm 0.024$						& 3.744													& $\boldsymbol{0.960\,(0.959) \pm 0.011}$					& $\boldsymbol{5.727}$										\\
																			& $^\ast$FedNorm+$^\ast$				& $0.940\,(0.947) \pm 0.029$						& 3.524													& $0.942\,(0.949) \pm 0.019$								& 3.744														\\
																			  \cdashline{3-6}
																			& $^\ast$Centralized$^\ast$				& $0.948\,(0.957) \pm 0.024$						& 4.405													& $0.944\,(0.951) \pm 0.027$								& 3.965														\\
			\midrule
			\multirow{8}{*}{\shortstack{SLIVER07\\(CT)}}					& Local									& $0.903\,(0.907) \pm 0.075$						& -														& $0.903\,(0.907) \pm 0.075$								& -	 														\\
																			  \cdashline{3-6}
																			& FedAvg								& $0.908\,(0.932) \pm 0.086$						& 0.554													& $0.841\,(0.924) \pm 0.251$								& -6.866													\\
																			& $^\ast$FedAvgM						& $0.742\,(0.749) \pm 0.061$						& -17.829												& $0.842\,(0.865) \pm 0.072$								& -6.755													\\
																			& FedVC$^\ast$							& $0.872\,(0.900) \pm 0.102$						& -3.433												& $0.761\,(0.799) \pm 0.147$								& -15.725													\\
																			& SiloBN								& $0.923\,(0.936) \pm 0.052$						& 2.215													& $0.913\,(0.941) \pm 0.071$								& 1.107														\\
																			& FedBN									& $0.920\,(0.930) \pm 0.053$						& 1.883													& $0.932\,(0.941) \pm 0.047$								& 3.212														\\
																			& FedNorm								& $\boldsymbol{0.940\,(0.954) \pm 0.056}$			& $\boldsymbol{4.097}$									& $0.914\,(0.944) \pm 0.096$								& 1.218														\\
																			& FedNorm+								& $0.935\,(0.941) \pm 0.053$						& 3.544													& $\boldsymbol{0.936\,(0.946) \pm 0.040}$					& $\boldsymbol{3.654}$										\\
																			  \cdashline{3-6}
																			& Centralized							& $0.922\,(0.944) \pm 0.084$						& 2.104													& $0.906\,(0.948) \pm 0.104$								& 0.332														\\
			\midrule
			\multirow{8}{*}{\shortstack{CHAOS19 MR\\T1 In-Phase\\(MRI)}}	& Local									& $0.724\,(0.825) \pm 0.287$						& -														& $0.724\,(0.825) \pm 0.287$								& -	 														\\
																			  \cdashline{3-6}
																			& $^\ast$FedAvg							& $0.106\,(0.060) \pm 0.119$						& -85.359												& $0.431\,(0.495) \pm 0.285$								& -40.47													\\
																			& $^\ast$FedAvgM						& $0.021\,(0.004) \pm 0.032$						& -97.099												& $0.638\,(0.771) \pm 0.289$								& -11.878													\\
																			& $^\ast$FedVC							& $0.090\,(0.040) \pm 0.124$						& -87.569												& $0.650\,(0.788) \pm 0.296$								& -10.221													\\
																			& $^\ast$SiloBN							& $0.189\,(0.079) \pm 0.252$						& -73.895												& $0.583\,(0.750) \pm 0.302$								& -19.475													\\
																			& $^\ast$FedBN$^\ast$					& $0.180\,(0.023) \pm 0.304$						& -75.138												& $0.194\,(0.046) \pm 0.302$								& -73.204													\\
																			& FedNorm								& $\boldsymbol{0.469\,(0.511) \pm 0.231}$			& $\boldsymbol{-35.221}$								& $\boldsymbol{0.791\,(0.810) \pm 0.104}$					& $\boldsymbol{9.254}$										\\
																			& $^\ast$FedNorm+$^\ast$				& $0.067\,(0.043) \pm 0.075$						& -90.746												& $0.230\,(0.196) \pm 0.215$								& -68.232													\\
																			  \cdashline{3-6}
																			& Centralized							& $0.618\,(0.739) \pm 0.329$						& -14.641												& $0.712\,(0.896) \pm 0.334$								& -1.657													\\
			\midrule
			\multirow{8}{*}{\shortstack{CHAOS19 MR\\T1 Out-Phase\\(MRI)}}	& Local									& -													& -														& $0.750\,(0.795) \pm 0.138$								& -	 														\\
																			  \cdashline{3-6}
																			& FedAvg$^\ast$							& \multirow{7}{*}{-}								& \multirow{7}{*}{-}									& $0.467\,(0.553) \pm 0.270$								& -37.733													\\
																			& FedAvgM								& 													& 														& $0.700\,(0.791) \pm 0.213$								& -6.667													\\
																			& FedVC									& 													& 														& $0.673\,(0.788) \pm 0.291$								& -10.267													\\
																			& SiloBN								& 													& 														& $0.686\,(0.740) \pm 0.237$								& -8.533													\\
																			& FedBN									& 													& 														& $0.457\,(0.610) \pm 0.381$								& -39.067													\\
																			& FedNorm								& 													& 														& $\boldsymbol{0.755\,(0.767) \pm 0.100}$					& $\boldsymbol{0.667}$										\\
																			& FedNorm+$^\ast$						&													&														& $0.253\,(0.173) \pm 0.265$								& -66.267													\\
																			  \cdashline{3-6}
																			& Centralized							& -													& -														& $0.729\,(0.858) \pm 0.315$								& -2.8														\\
			\midrule
			\multirow{8}{*}{\shortstack{CHAOS19 MR\\T1 Water\\(MRI)}}		& Local									& -													& -														& $0.646\,(0.760) \pm 0.266$								& -	 														\\
																			  \cdashline{3-6}
																			& FedAvg								& \multirow{7}{*}{-}								& \multirow{7}{*}{-}									& $0.451\,(0.530) \pm 0.291$								& -30.186													\\
																			& FedAvgM								& 													& 														& $0.700\,(0.809) \pm 0.254$								& 8.359														\\
																			& FedVC									& 													& 														& $0.690\,(0.821) \pm 0.302$								& 6.811														\\
																			& SiloBN								& 													& 														& $0.717\,(0.742) \pm 0.185$								& 10.991													\\
																			& FedBN									& 													& 														& $0.533\,(0.647) \pm 0.350$								& -17.492													\\
																			& FedNorm								& 													& 														& $\boldsymbol{0.799\,(0.808) \pm 0.090}$					& $\boldsymbol{23.684}$										\\
																			& FedNorm+$^\ast$						&													&														& $0.288\,(0.172) \pm 0.318$								& -55.418													\\
																			  \cdashline{3-6}
																			& Centralized							& -													& -														& $0.738\,(0.891) \pm 0.316$								& 14.241													\\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
\end{table*}

==> tables/comparison-non-iid-3-old.tex <==
% !TeX root = ../main.tex
% Add the above to each chapter to make compiling the PDF easier in some editors.
\begin{table*}[ht]
	\caption[Comparison: Non-IID 3 Setting]{Comparison of methods for the Non-IID 3 setting. The results give the performance of the local models, the learned global model, and the centralized model on the test set of each client. The relative improvement based on \Cref{eqn:relative-improvement} is given for the scores of the FL methods and the centralized model over local model for the mean Dice per patient. A star ($^\ast$) behind the method name indicates that the results are statistically significant compared to the local model for a $p$-value $\leq 0.05$ using the two-sided t-test. The best performance for each column per client is highlighted in bold.}\label{tab:comparison-non-iid-3}
	\centering
	\begin{adjustbox}{max width=\textwidth, max height=0.45\textheight}
		\begin{tabular}{c c c c c c c c c}
			\toprule
			\textbf{Client}																	& \multirow{2}{*}{\textbf{Methods}}	& \textbf{Dice per}										& \textbf{Relative}								& \textbf{VOE per}								& \textbf{RVD per}											& \textbf{ASSD per}								& \textbf{MSSD per}								& \textbf{RMSD per}								\\
			\textbf{(Modality)}																&									& \textbf{Patient} $\boldsymbol{\uparrow}$				& \textbf{Impr. (\%)} $\boldsymbol{\uparrow}$	& \textbf{Patient} $\boldsymbol{\downarrow}$	& \textbf{Patient} $\lvert\boldsymbol{\downarrow}\rvert$	& \textbf{Patient} $\boldsymbol{\downarrow}$	& \textbf{Patient} $\boldsymbol{\downarrow}$	& \textbf{Patient} $\boldsymbol{\downarrow}$	\\
			\midrule
			\multirow{7}{*}{\shortstack{Multi-Atlas\\(CT)}}									& Local								& $0.867\,(0.889) \pm 0.061$							& -												& $22.997\,(19.932) \pm 9.004$					& $0.486\,(-0.958) \pm 13.367$								& $14.514\,(10.877) \pm 10.516$					& $246.672\,(249.636) \pm 79.353$				& $39.664\,(32.768) \pm 23.412$					\\
																							  \cdashline{2-9}
																							& FedAvg$^\ast$						& $0.924\,(0.934) \pm 0.027$							& 6.574											& $13.956\,(12.376) \pm 4.547$					& $5.227\,(2.843) \pm 6.535$								& $8.513\,(5.459) \pm 8.576$					& $\boldsymbol{185.746\,(195.502) \pm 84.609}$	& $25.276\,(22.650) \pm 19.756$					\\
																							& FedVC								& $0.886\,(0.892) \pm 0.048$							& 2.191											& $20.148\,(19.534) \pm 7.276$					& $14.514\,(9.279) \pm 13.763$								& $22.128\,(17.728) \pm 14.044$					& $265.621\,(272.171) \pm 72.206$				& $57.381\,(57.290) \pm 26.768$					\\
																							& SiloBN							& $0.889\,(0.896) \pm 0.051$							& 2.537											& $19.688\,(18.868) \pm 7.729$					& $13.531\,(10.232) \pm 15.476$								& $19.248\,(18.988) \pm 11.575$					& $252.962\,(266.030) \pm 70.852$				& $47.721\,(53.028) \pm 23.372$					\\
																							& FedBN								& $0.899\,(0.932) \pm 0.073$							& 3.691											& $17.593\,(12.677) \pm 10.911$					& $10.117\,(3.009) \pm 19.255$								& $18.520\,(9.199) \pm 22.221$					& $243.926\,(266.729) \pm 67.123$				& $43.453\,(37.715) \pm 35.544$					\\
																							& FedNorm+$^\ast$					& $\boldsymbol{0.931\,(0.939) \pm 0.025}$				& $\boldsymbol{7.382}$							& $\boldsymbol{12.859\,(11.464) \pm 4.246}$		& $\boldsymbol{3.055\,(2.849) \pm 5.965}$					& $\boldsymbol{5.786\,(3.926) \pm 5.959}$		& $227.878\,(230.931) \pm 87.757$				& $\boldsymbol{20.149\,(16.744) \pm 14.318}$	\\
																							  \cdashline{2-9}
																							& Centralized$^\ast$				& $0.927\,(0.941) \pm 0.030$							& 6.920											& $13.456\,(11.212) \pm 5.007$					& $4.302\,(2.064) \pm 7.356$								& $8.358\,(7.537) \pm 6.542$					& $240.652\,(239.207) \pm 78.120$				& $28.515\,(26.397) \pm 18.145$					\\
			\midrule		
			\multirow{7}{*}{\shortstack{3D-IRCADb\\(CT)}}									& Local								& $0.908\,(0.914) \pm 0.026$							& -												& $16.775\,(15.822) \pm 4.310$					& $-6.095\,(-6.293) \pm 2.482$								& $4.117\,(3.654) \pm 1.211$					& $111.923\,(115.828) \pm 29.781$				& $9.188\,(9.488) \pm 2.852$					\\
																							  \cdashline{2-9}
																							& FedAvg							& $0.926\,(0.942) \pm 0.040$							& 1.982											& $13.640\,(11.052) \pm 6.460$					& $3.107\,(2.634) \pm 2.748$								& $4.304\,(3.458) \pm 1.868$					& $81.556\,(78.512) \pm 26.809$					& $9.821\,(8.855) \pm 4.094$					\\
																							& FedVC								& $0.915\,(0.928) \pm 0.039$							& 0.771											& $15.426\,(13.346) \pm 6.260$					& $8.865\,(7.635) \pm 4.692$								& $5.106\,(4.745) \pm 2.093$					& $96.589\,(90.853) \pm 30.490$					& $11.367\,(10.596) \pm 3.935$					\\
																							& SiloBN$^\ast$						& $0.948\,(0.958) \pm 0.027$							& 4.405											& $9.762\,(8.010) \pm 4.667$					& $\boldsymbol{-0.616\,(-0.571) \pm 2.547}$					& $2.550\,(2.246) \pm 1.195$					& $\boldsymbol{64.955\,(54.196) \pm 28.794}$	& $6.074\,(5.834) \pm 2.194$					\\
																							& FedBN$^\ast$						& $0.941\,(0.953) \pm 0.031$							& 3.634											& $10.993\,(8.936) \pm 5.327$					& $-1.056\,(-0.516) \pm 3.415$								& $2.751\,(2.408) \pm 1.266$					& $68.230\,(61.943) \pm 29.922$					& $6.024\,(4.609) \pm 3.055$					\\
																							& FedNorm+$^\ast$					& $0.948\,(0.949) \pm 0.016$							& 4.405											& $9.863\,(9.619) \pm 2.822$					& $2.313\,(1.316) \pm 2.836$								& $\boldsymbol{2.515\,(2.430) \pm 0.917}$		& $70.544\,(64.626) \pm 21.659$					& $\boldsymbol{5.861\,(5.721) \pm 1.133}$		\\
																							  \cdashline{2-9}
																							& Centralized$^\ast$				& $\boldsymbol{0.956\,(0.960) \pm 0.015}$				& $\boldsymbol{5.286}$							& $\boldsymbol{8.321\,(7.782) \pm 2.635}$		& $1.551\,(1.408) \pm 2.016$								& $2.802\,(2.671) \pm 1.038$					& $128.130\,(126.828) \pm 24.221$				& $8.896\,(8.834) \pm 2.534$					\\
			\midrule
			\multirow{7}{*}{\shortstack{CHAOS19 MR\\T1 Water\\(MRI)}}						& Local								& $0.646\,(0.760) \pm 0.266$							& -												& $48.024\,(38.696) \pm 25.224$					& $-34.489\,(-24.830) \pm 30.415$							& $12.316\,(7.716) \pm 10.823$					& $96.891\,(106.341) \pm 34.801$				& $20.208\,(16.136) \pm 12.732$					\\
																							  \cdashline{2-9}
																							& FedAvg							& $0.468\,(0.512) \pm 0.334$							& -27.554										& $63.837\,(63.958) \pm 29.651$					& $-44.152\,(-54.709) \pm 50.369$							& $25.196\,(26.954) \pm 15.814$					& $\boldsymbol{136.788\,(130.043) \pm 64.780}$	& $38.604\,(41.959) \pm 21.507$					\\
																							& FedVC$^\ast$						& $0.314\,(0.242) \pm 0.323$							& -51.393										& $77.255\,(85.049) \pm 24.901$					& $\boldsymbol{-7.663\,(-37.268) \pm 116.082}$				& $55.768\,(50.822) \pm 44.521$					& $197.869\,(204.864) \pm 56.788$				& $69.909\,(66.392) \pm 41.981$					\\
																							& SiloBN							& $0.609\,(0.652) \pm 0.223$							& -5.728										& $52.981\,(51.392) \pm 22.902$					& $-22.924\,(-37.924) \pm 47.017$							& $15.534\,(16.318) \pm 4.755$					& $152.773\,(135.178) \pm 53.880$				& $27.636\,(25.823) \pm 8.127$					\\
																							& FedBN								& $0.563\,(0.631) \pm 0.332$							& -12.848										& $54.669\,(53.161) \pm 30.632$					& $-30.432\,(-35.151) \pm 52.540$							& $17.574\,(16.028) \pm 13.625$					& $137.522\,(134.657) \pm 36.964$				& $27.510\,(26.864) \pm 14.142$					\\
																							& FedNorm+							& $0.779\,(0.805) \pm 0.094$							& 20.588										& $35.459\,(32.588) \pm 11.871$					& $25.367\,(10.032) \pm 41.965$								& $14.647\,(11.289) \pm 8.307$					& $152.137\,(140.816) \pm 59.228$				& $30.544\,(26.158) \pm 12.529$					\\
																							  \cdashline{2-9}
																							& Centralized						& $\boldsymbol{0.826\,(0.873) \pm 0.090}$				& $\boldsymbol{27.864}$							& $\boldsymbol{28.877\,(22.498) \pm 12.339}$	& $9.192\,(0.136) \pm 23.564$								& $\boldsymbol{10.838\,(7.143) \pm 6.728}$		& $142.285\,(129.159) \pm 58.372$				& $\boldsymbol{25.875\,(18.385) \pm 14.797}$	\\
			\midrule		
			\multirow{7}{*}{\shortstack{KORA\\T1 Water (1)\\(MRI)}}							& Local								& $0.864\,(0.859) \pm 0.054$							& -												& $23.613\,(24.739) \pm 8.262$					& $8.859\,(8.213) \pm 10.202$								& $10.334\,(8.798) \pm 6.262$					& $103.790\,(111.421) \pm 23.178$				& $20.273\,(19.345) \pm 10.280$					\\
																							  \cdashline{2-9}
																							& FedAvg$^\ast$						& $0.924\,(0.936) \pm 0.034$							& 6.944											& $13.910\,(12.022) \pm 5.711$					& $-6.664\,(-6.359) \pm 4.827$								& $3.628\,(2.587) \pm 2.955$					& $65.260\,(39.347) \pm 52.066$					& $8.065\,(5.503) \pm 8.359$					\\
																							& FedVC$^\ast$						& $0.920\,(0.914) \pm 0.025$							& 6.481											& $14.752\,(15.837) \pm 4.315$					& $2.566\,(2.705) \pm 6.040$								& $4.456\,(3.166) \pm 3.030$					& $86.576\,(93.801) \pm 41.325$					& $10.121\,(6.217) \pm 8.546$					\\
																							& SiloBN$^\ast$						& $0.934\,(0.944) \pm 0.029$							& 8.102											& $12.203\,(10.562) \pm 4.994$					& $\boldsymbol{-0.975\,(-0.899) \pm 3.978}$					& $2.800\,(2.416) \pm 1.478$					& $59.242\,(50.328) \pm 44.540$					& $6.197\,(4.958) \pm 4.402$					\\
																							& FedBN$^\ast$						& $0.936\,(0.946) \pm 0.029$							& 8.333											& $11.954\,(10.203) \pm 4.991$					& $-5.064\,(-3.312) \pm 6.114$								& $\boldsymbol{2.411\,(1.989) \pm 1.005}$		& $\boldsymbol{51.431\,(43.221) \pm 26.661}$	& $\boldsymbol{4.470\,(3.301) \pm 2.186}$		\\
																							& FedNorm+$^\ast$					& $\boldsymbol{0.938\,(0.945) \pm 0.025}$				& $\boldsymbol{8.565}$							& $\boldsymbol{11.615\,(10.357) \pm 4.309}$		& $1.138\,(1.074) \pm 3.333$								& $3.356\,(2.978) \pm 2.153$					& $108.647\,(113.454) \pm 38.574$				& $8.718\,(7.925) \pm 4.990$					\\
																							  \cdashline{2-9}
																							& Centralized$^\ast$				& $0.936\,(0.944) \pm 0.025$							& 8.333											& $12.001\,(10.650) \pm 4.436$					& $-4.327\,(-3.595) \pm 4.264$								& $2.626\,(2.254) \pm 1.005$					& $70.333\,(62.346) \pm 37.758$					& $5.561\,(5.111) \pm 2.499$					\\
			\midrule
			\multirow{7}{*}{\shortstack{SLIVER07\\+ KORA T1\\Water (2)\\(CT + MRI)}}		& Local								& $0.726\,(0.900) \pm 0.352$							& -												& $34.327\,(18.204) \pm 33.661$					& $-22.187\,(-4.645) \pm 35.156$							& $15.491\,(6.364) \pm 18.592$					& $127.262\,(113.080) \pm 77.507$				& $24.471\,(11.123) \pm 23.901$					\\
																							  \cdashline{2-9}
																							& FedAvg							& $0.742\,(0.922) \pm 0.367$							& 2.204											& $31.461\,(14.506) \pm 35.221$					& $-24.541\,(-6.403) \pm 37.643$							& $14.063\,(4.723) \pm 20.883$					& $\boldsymbol{96.237\,(79.303) \pm 71.538}$	& $20.426\,(9.295) \pm 22.476$					\\
																							& FedVC								& $0.740\,(0.925) \pm 0.350$							& 1.928											& $32.416\,(13.870) \pm 34.374$					& $-19.992\,(-2.684) \pm 35.362$							& $11.757\,(5.338) \pm 14.151$					& $126.538\,(135.336) \pm 75.115$				& $19.366\,(9.357) \pm 17.923$					\\
																							& SiloBN							& $0.746\,(0.908) \pm 0.344$							& 2.755											& $31.968\,(16.890) \pm 33.485$					& $-14.034\,(-0.228) \pm 39.892$							& $16.681\,(9.308) \pm 16.002$					& $160.677\,(149.690) \pm 60.672$				& $29.135\,(18.418) \pm 24.511$					\\
																							& FedBN								& $0.745\,(0.933) \pm 0.369$							& 2.617											& $30.809\,(12.508) \pm 35.869$					& $-21.469\,(-3.070) \pm 38.915$							& $10.701\,(4.418) \pm 14.073$					& $114.511\,(83.127) \pm 79.430$				& $17.228\,(8.953) \pm 16.875$					\\
																							& FedNorm+							& $0.752\,(0.946) \pm 0.360$							& 3.581											& $30.148\,(10.334) \pm 35.665$					& $-22.677\,(-3.379) \pm 37.415$							& $9.703\,(3.446) \pm 12.815$					& $109.673\,(105.453) \pm 72.976$				& $\boldsymbol{15.722\,(9.647) \pm 15.727}$		\\
																							  \cdashline{2-9}
																							& Centralized						& $\boldsymbol{0.848\,(0.940) \pm 0.174}$				& $\boldsymbol{16.804}$							& $\boldsymbol{23.300\,(11.254) \pm 22.380}$	& $\boldsymbol{-7.912\,(-3.645) \pm 14.775}$				& $\boldsymbol{7.757\,(5.793) \pm 6.237}$		& $119.134\,(93.511) \pm 81.877$				& $17.012\,(13.547) \pm 14.533$					\\
			\midrule		
			\multirow{7}{*}{\shortstack{LiTS17\\Site 2\\+ KORA T1\\Water (3)\\(CT + MRI)}}	& Local								& $0.879\,(0.917) \pm 0.093$							& -												& $20.647\,(15.247) \pm 13.131$					& $-0.321\,(2.877) \pm 16.538$								& $10.711\,(6.939) \pm 9.084$					& $187.841\,(150.326) \pm 100.611$				& $26.217\,(21.219) \pm 20.777$					\\
																							  \cdashline{2-9}
																							& FedAvg							& $0.920\,(0.952) \pm 0.083$							& 4.664											& $14.005\,(9.202) \pm 12.065$					& $-4.890\,(-1.600) \pm 14.333$								& $4.845\,(2.310) \pm 4.997$					& $123.582\,(82.451) \pm 109.102$				& $12.770\,(7.807) \pm 15.309$					\\
																							& FedVC								& $0.901\,(0.929) \pm 0.089$							& 2.503											& $17.038\,(13.230) \pm 12.368$					& $-1.662\,(0.961) \pm 16.111$								& $11.221\,(10.214) \pm 9.436$					& $179.557\,(147.417) \pm 112.612$				& $30.167\,(25.485) \pm 27.076$					\\
																							& SiloBN$^\ast$						& $0.937\,(0.953) \pm 0.039$							& 6.598											& $11.655\,(8.987) \pm 6.649$					& $\boldsymbol{-0.696\,(-0.740) \pm 9.044}$					& $5.884\,(2.510) \pm 7.760$					& $145.176\,(119.342) \pm 106.814$				& $16.287\,(7.035) \pm 20.742$					\\
																							& FedBN								& $0.935\,(0.952) \pm 0.048$							& 6.371											& $11.933\,(9.122) \pm 7.901$					& $-3.939\,(-1.675) \pm 9.959$								& $3.366\,(2.485) \pm 2.900$					& $118.912\,(80.751) \pm 85.408$				& $9.623\,(6.214) \pm 10.548$					\\
																							& FedNorm+$^\ast$					& $\boldsymbol{0.947\,(0.952) \pm 0.023}$				& $\boldsymbol{7.736}$							& $\boldsymbol{9.956\,(9.136) \pm 3.987}$		& $-1.199\,(0.365) \pm 5.746$								& $\boldsymbol{2.848\,(2.303) \pm 1.579}$		& $\boldsymbol{112.673\,(72.614) \pm 89.356}$	& $\boldsymbol{8.299\,(7.447) \pm 7.030}$		\\
																							  \cdashline{2-9}
																							& Centralized$^\ast$				& $0.944\,(0.954) \pm 0.023$							& 7.395											& $10.465\,(8.849) \pm 4.035$					& $-1.005\,(-1.091) \pm 5.035$								& $5.583\,(3.116) \pm 5.779$					& $166.922\,(146.448) \pm 116.774$				& $17.615\,(7.974) \pm 19.005$					\\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
\end{table*}

==> tables/comparison-non-iid-3.tex <==
% !TeX root = ../main.tex
% Add the above to each chapter to make compiling the PDF easier in some editors.
\begin{table*}[ht]
	\caption[Comparison: Non-IID 3 Setting]{\todo{Add Non-IID 2 results, only Dice and RI} Comparison on the Non-IID 3 setting. The numbers give the performances of the local models, the centralized model, and the
											federated global models (without refinement at the clients) on the test set of each client. \fedavgm and \fednorm
											are not included in this table because \fedavgm fails during training in this setting and \fednorm cannot handle
											mixed-modality clients. The performances are reported with Dice, VOE, ASSD, MSSD, and RMSD per patient and are given
											by mean (median) and standard deviation. Additionally, the RI is computed
											for the mean Dice per patient of the models from the FL algorithms and the centralized model over the local model
											performance. Hence, the RI is not reported for the local models. The best score from the federated models per metric and client is highlighted
											in bold. A star ($^\ast$) after the method name indicates that the results are statistically significant
											with a $p$-value $\leq 0.05$ using the unpaired two-sided t-test on the Dice per patient scores from the local model
											and the respective federated/centralized model.}\label{tab:comparison-non-iid-3}
	\centering
	\begin{adjustbox}{max width=\textwidth, max height=0.45\textheight}
		\begin{tabular}{c l c c c c c c}
			\toprule
			\textbf{Client}																	& \multirow{2}{*}{\textbf{Methods}}	& \textbf{Dice per}										& \textbf{RI} $\boldsymbol{\uparrow}$			& \textbf{VOE per}								& \textbf{ASSD per}								& \textbf{MSSD per}								& \textbf{RMSD per}								\\
			\textbf{(Modality)}																&									& \textbf{Patient} $\boldsymbol{\uparrow}$				& \textbf{[\%]} 								& \textbf{Patient} $\boldsymbol{\downarrow}$	& \textbf{Patient} $\boldsymbol{\downarrow}$	& \textbf{Patient} $\boldsymbol{\downarrow}$	& \textbf{Patient} $\boldsymbol{\downarrow}$	\\
			\midrule
			\multirow{7}{*}{\shortstack{Multi-Atlas\\(CT)}}									& Local								& $0.867\,(0.889) \pm 0.061$							& -												& $22.997\,(19.932) \pm 9.004$					& $14.514\,(10.877) \pm 10.516$					& $246.672\,(249.636) \pm 79.353$				& $39.664\,(32.768) \pm 23.412$					\\
																							  \cdashline{2-8}
																							& FedAvg$^\ast$~\cite{FedAvg}		& $0.924\,(0.934) \pm 0.027$							& 6.574											& $13.956\,(12.376) \pm 4.547$					& $8.513\,(5.459) \pm 8.576$					& $\boldsymbol{185.746\,(195.502) \pm 84.609}$	& $25.276\,(22.650) \pm 19.756$					\\
																							& FedVC~\cite{FedVC}				& $0.886\,(0.892) \pm 0.048$							& 2.191											& $20.148\,(19.534) \pm 7.276$					& $22.128\,(17.728) \pm 14.044$					& $265.621\,(272.171) \pm 72.206$				& $57.381\,(57.290) \pm 26.768$					\\
																							& SiloBN~\cite{SiloBN}				& $0.889\,(0.896) \pm 0.051$							& 2.537											& $19.688\,(18.868) \pm 7.729$					& $19.248\,(18.988) \pm 11.575$					& $252.962\,(266.030) \pm 70.852$				& $47.721\,(53.028) \pm 23.372$					\\
																							& FedBN~\cite{FedBN}				& $0.899\,(0.932) \pm 0.073$							& 3.691											& $17.593\,(12.677) \pm 10.911$					& $18.520\,(9.199) \pm 22.221$					& $243.926\,(266.729) \pm 67.123$				& $43.453\,(37.715) \pm 35.544$					\\
																							& FedNorm+$^\ast$					& $\boldsymbol{0.931\,(0.939) \pm 0.025}$				& $\boldsymbol{7.382}$							& $\boldsymbol{12.859\,(11.464) \pm 4.246}$		& $\boldsymbol{5.786\,(3.926) \pm 5.959}$		& $227.878\,(230.931) \pm 87.757$				& $\boldsymbol{20.149\,(16.744) \pm 14.318}$	\\
																							  \cdashline{2-8}
																							& Centralized$^\ast$				& $0.927\,(0.941) \pm 0.030$							& 6.920											& $13.456\,(11.212) \pm 5.007$					& $8.358\,(7.537) \pm 6.542$					& $240.652\,(239.207) \pm 78.120$				& $28.515\,(26.397) \pm 18.145$					\\
			\midrule		
			\multirow{7}{*}{\shortstack{3D-IRCADb\\(CT)}}									& Local								& $0.908\,(0.914) \pm 0.026$							& -												& $16.775\,(15.822) \pm 4.310$					& $4.117\,(3.654) \pm 1.211$					& $111.923\,(115.828) \pm 29.781$				& $9.188\,(9.488) \pm 2.852$					\\
																							  \cdashline{2-8}
																							& FedAvg~\cite{FedAvg}				& $0.926\,(0.942) \pm 0.040$							& 1.982											& $13.640\,(11.052) \pm 6.460$					& $4.304\,(3.458) \pm 1.868$					& $81.556\,(78.512) \pm 26.809$					& $9.821\,(8.855) \pm 4.094$					\\
																							& FedVC~\cite{FedVC}				& $0.915\,(0.928) \pm 0.039$							& 0.771											& $15.426\,(13.346) \pm 6.260$					& $5.106\,(4.745) \pm 2.093$					& $96.589\,(90.853) \pm 30.490$					& $11.367\,(10.596) \pm 3.935$					\\
																							& SiloBN$^\ast$~\cite{SiloBN}		& $\boldsymbol{0.948\,(0.958) \pm 0.027}$				& $\boldsymbol{4.405}$							& $\boldsymbol{9.762\,(8.010) \pm 4.667}$		& $2.550\,(2.246) \pm 1.195$					& $\boldsymbol{64.955\,(54.196) \pm 28.794}$	& $6.074\,(5.834) \pm 2.194$					\\
																							& FedBN$^\ast$~\cite{FedBN}		& $0.941\,(0.953) \pm 0.031$							& 3.634											& $10.993\,(8.936) \pm 5.327$					& $2.751\,(2.408) \pm 1.266$					& $68.230\,(61.943) \pm 29.922$					& $6.024\,(4.609) \pm 3.055$					\\
																							& FedNorm+$^\ast$					& $\boldsymbol{0.948\,(0.949) \pm 0.016}$				& $\boldsymbol{4.405}$							& $9.863\,(9.619) \pm 2.822$					& $\boldsymbol{2.515\,(2.430) \pm 0.917}$		& $70.544\,(64.626) \pm 21.659$					& $\boldsymbol{5.861\,(5.721) \pm 1.133}$		\\
																							  \cdashline{2-8}
																							& Centralized$^\ast$				& $0.956\,(0.960) \pm 0.015$							& 5.286											& $8.321\,(7.782) \pm 2.635$					& $2.802\,(2.671) \pm 1.038$					& $128.130\,(126.828) \pm 24.221$				& $8.896\,(8.834) \pm 2.534$					\\
			\midrule
			\multirow{7}{*}{\shortstack{CHAOS19 MR\\T1 Water\\(MRI)}}						& Local								& $0.646\,(0.760) \pm 0.266$							& -												& $48.024\,(38.696) \pm 25.224$					& $12.316\,(7.716) \pm 10.823$					& $96.891\,(106.341) \pm 34.801$				& $20.208\,(16.136) \pm 12.732$					\\
																							  \cdashline{2-8}
																							& FedAvg~\cite{FedAvg}				& $0.468\,(0.512) \pm 0.334$							& -27.554										& $63.837\,(63.958) \pm 29.651$					& $25.196\,(26.954) \pm 15.814$					& $\boldsymbol{136.788\,(130.043) \pm 64.780}$	& $38.604\,(41.959) \pm 21.507$					\\
																							& FedVC$^\ast$~\cite{FedVC}		& $0.314\,(0.242) \pm 0.323$							& -51.393										& $77.255\,(85.049) \pm 24.901$					& $55.768\,(50.822) \pm 44.521$					& $197.869\,(204.864) \pm 56.788$				& $69.909\,(66.392) \pm 41.981$					\\
																							& SiloBN~\cite{SiloBN}				& $0.609\,(0.652) \pm 0.223$							& -5.728										& $52.981\,(51.392) \pm 22.902$					& $15.534\,(16.318) \pm 4.755$					& $152.773\,(135.178) \pm 53.880$				& $27.636\,(25.823) \pm 8.127$					\\
																							& FedBN~\cite{FedBN}				& $0.563\,(0.631) \pm 0.332$							& -12.848										& $54.669\,(53.161) \pm 30.632$					& $17.574\,(16.028) \pm 13.625$					& $137.522\,(134.657) \pm 36.964$				& $\boldsymbol{27.510\,(26.864) \pm 14.142}$	\\
																							& FedNorm+							& $\boldsymbol{0.779\,(0.805) \pm 0.094}$				& $\boldsymbol{20.588}$							& $\boldsymbol{35.459\,(32.588) \pm 11.871}$	& $\boldsymbol{14.647\,(11.289) \pm 8.307}$		& $152.137\,(140.816) \pm 59.228$				& $30.544\,(26.158) \pm 12.529$					\\
																							  \cdashline{2-8}
																							& Centralized						& $0.826\,(0.873) \pm 0.090$							& 27.864										& $28.877\,(22.498) \pm 12.339$					& $10.838\,(7.143) \pm 6.728$					& $142.285\,(129.159) \pm 58.372$				& $25.875\,(18.385) \pm 14.797$					\\
			\midrule		
			\multirow{7}{*}{\shortstack{KORA\\T1 Water (1)\\(MRI)}}							& Local								& $0.864\,(0.859) \pm 0.054$							& -												& $23.613\,(24.739) \pm 8.262$					& $10.334\,(8.798) \pm 6.262$					& $103.790\,(111.421) \pm 23.178$				& $20.273\,(19.345) \pm 10.280$					\\
																							  \cdashline{2-8}
																							& FedAvg$^\ast$~\cite{FedAvg}		& $0.924\,(0.936) \pm 0.034$							& 6.944											& $13.910\,(12.022) \pm 5.711$					& $3.628\,(2.587) \pm 2.955$					& $65.260\,(39.347) \pm 52.066$					& $8.065\,(5.503) \pm 8.359$					\\
																							& FedVC$^\ast$~\cite{FedVC}		& $0.920\,(0.914) \pm 0.025$							& 6.481											& $14.752\,(15.837) \pm 4.315$					& $4.456\,(3.166) \pm 3.030$					& $86.576\,(93.801) \pm 41.325$					& $10.121\,(6.217) \pm 8.546$					\\
																							& SiloBN$^\ast$~\cite{SiloBN}		& $0.934\,(0.944) \pm 0.029$							& 8.102											& $12.203\,(10.562) \pm 4.994$					& $2.800\,(2.416) \pm 1.478$					& $59.242\,(50.328) \pm 44.540$					& $6.197\,(4.958) \pm 4.402$					\\
																							& FedBN$^\ast$~\cite{FedBN}		& $0.936\,(0.946) \pm 0.029$							& 8.333											& $11.954\,(10.203) \pm 4.991$					& $\boldsymbol{2.411\,(1.989) \pm 1.005}$		& $\boldsymbol{51.431\,(43.221) \pm 26.661}$	& $\boldsymbol{4.470\,(3.301) \pm 2.186}$		\\
																							& FedNorm+$^\ast$					& $\boldsymbol{0.938\,(0.945) \pm 0.025}$				& $\boldsymbol{8.565}$							& $\boldsymbol{11.615\,(10.357) \pm 4.309}$		& $3.356\,(2.978) \pm 2.153$					& $108.647\,(113.454) \pm 38.574$				& $8.718\,(7.925) \pm 4.990$					\\
																							  \cdashline{2-8}
																							& Centralized$^\ast$				& $0.936\,(0.944) \pm 0.025$							& 8.333											& $12.001\,(10.650) \pm 4.436$					& $2.626\,(2.254) \pm 1.005$					& $70.333\,(62.346) \pm 37.758$					& $5.561\,(5.111) \pm 2.499$					\\
			\midrule
			\multirow{7}{*}{\shortstack{SLIVER07\\+ KORA T1\\Water (2)\\(CT + MRI)}}		& Local								& $0.726\,(0.900) \pm 0.352$							& -												& $34.327\,(18.204) \pm 33.661$					& $15.491\,(6.364) \pm 18.592$					& $127.262\,(113.080) \pm 77.507$				& $24.471\,(11.123) \pm 23.901$					\\
																							  \cdashline{2-8}
																							& FedAvg~\cite{FedAvg}				& $0.742\,(0.922) \pm 0.367$							& 2.204											& $31.461\,(14.506) \pm 35.221$					& $14.063\,(4.723) \pm 20.883$					& $\boldsymbol{96.237\,(79.303) \pm 71.538}$	& $20.426\,(9.295) \pm 22.476$					\\
																							& FedVC~\cite{FedVC}				& $0.740\,(0.925) \pm 0.350$							& 1.928											& $32.416\,(13.870) \pm 34.374$					& $11.757\,(5.338) \pm 14.151$					& $126.538\,(135.336) \pm 75.115$				& $19.366\,(9.357) \pm 17.923$					\\
																							& SiloBN~\cite{SiloBN}				& $0.746\,(0.908) \pm 0.344$							& 2.755											& $31.968\,(16.890) \pm 33.485$					& $16.681\,(9.308) \pm 16.002$					& $160.677\,(149.690) \pm 60.672$				& $29.135\,(18.418) \pm 24.511$					\\
																							& FedBN~\cite{FedBN}				& $0.745\,(0.933) \pm 0.369$							& 2.617											& $30.809\,(12.508) \pm 35.869$					& $10.701\,(4.418) \pm 14.073$					& $114.511\,(83.127) \pm 79.430$				& $17.228\,(8.953) \pm 16.875$					\\
																							& FedNorm+							& $\boldsymbol{0.752\,(0.946) \pm 0.360}$				& $\boldsymbol{3.581}$							& $\boldsymbol{30.148\,(10.334) \pm 35.665}$	& $\boldsymbol{9.703\,(3.446) \pm 12.815}$		& $109.673\,(105.453) \pm 72.976$				& $\boldsymbol{15.722\,(9.647) \pm 15.727}$		\\
																							  \cdashline{2-8}
																							& Centralized						& $0.848\,(0.940) \pm 0.174$							& 16.804										& $23.300\,(11.254) \pm 22.380$					& $7.757\,(5.793) \pm 6.237$					& $119.134\,(93.511) \pm 81.877$				& $17.012\,(13.547) \pm 14.533$					\\
			\midrule		
			\multirow{7}{*}{\shortstack{LiTS17\\Site 2\\+ KORA T1\\Water (3)\\(CT + MRI)}}	& Local								& $0.879\,(0.917) \pm 0.093$							& -												& $20.647\,(15.247) \pm 13.131$					& $10.711\,(6.939) \pm 9.084$					& $187.841\,(150.326) \pm 100.611$				& $26.217\,(21.219) \pm 20.777$					\\
																							  \cdashline{2-8}
																							& FedAvg~\cite{FedAvg}				& $0.920\,(0.952) \pm 0.083$							& 4.664											& $14.005\,(9.202) \pm 12.065$					& $4.845\,(2.310) \pm 4.997$					& $123.582\,(82.451) \pm 109.102$				& $12.770\,(7.807) \pm 15.309$					\\
																							& FedVC~\cite{FedVC}				& $0.901\,(0.929) \pm 0.089$							& 2.503											& $17.038\,(13.230) \pm 12.368$					& $11.221\,(10.214) \pm 9.436$					& $179.557\,(147.417) \pm 112.612$				& $30.167\,(25.485) \pm 27.076$					\\
																							& SiloBN$^\ast$~\cite{SiloBN}		& $0.937\,(0.953) \pm 0.039$							& 6.598											& $11.655\,(8.987) \pm 6.649$					& $5.884\,(2.510) \pm 7.760$					& $145.176\,(119.342) \pm 106.814$				& $16.287\,(7.035) \pm 20.742$					\\
																							& FedBN~\cite{FedBN}				& $0.935\,(0.952) \pm 0.048$							& 6.371											& $11.933\,(9.122) \pm 7.901$					& $3.366\,(2.485) \pm 2.900$					& $118.912\,(80.751) \pm 85.408$				& $9.623\,(6.214) \pm 10.548$					\\
																							& FedNorm+$^\ast$					& $\boldsymbol{0.947\,(0.952) \pm 0.023}$				& $\boldsymbol{7.736}$							& $\boldsymbol{9.956\,(9.136) \pm 3.987}$		& $\boldsymbol{2.848\,(2.303) \pm 1.579}$		& $\boldsymbol{112.673\,(72.614) \pm 89.356}$	& $\boldsymbol{8.299\,(7.447) \pm 7.030}$		\\
																							  \cdashline{2-8}
																							& Centralized$^\ast$				& $0.944\,(0.954) \pm 0.023$							& 7.395											& $10.465\,(8.849) \pm 4.035$					& $5.583\,(3.116) \pm 5.779$					& $166.922\,(146.448) \pm 116.774$				& $17.615\,(7.974) \pm 19.005$					\\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
\end{table*}

==> tables/model-selection-fednorm+.tex <==
% !TeX root = ../main.tex
% Add the above to each chapter to make compiling the PDF easier in some editors.
\begin{table}[ht]
	\caption[Model Selection: FedNorm+]{Highest global validation Dice scores for \fednormp with different interpolation ratios $\beta$ reported within 100 FL rounds
										of training. The best (overall highest) global validation Dice score in the table is highlighted in bold.}\label{tab:model-selection-fednormp}
	\centering
	\begin{tabular}{c c c c}
		\toprule
		\multicolumn{4}{c}{\textbf{Interpolation Ratio} $\boldsymbol{(\beta)}$}	\\
		\textbf{1.0}	& \textbf{0.9}		& \textbf{0.5}	& \textbf{0.2}		\\
		\midrule
		0.878			& $\mathbf{0.881}$	& 0.876			& 0.859				\\
		\bottomrule
	\end{tabular}
\end{table}

==> tables/model-selection-fednorm.tex <==
% !TeX root = ../main.tex
% Add the above to each chapter to make compiling the PDF easier in some editors.
\begin{table}[ht]
	\caption[Model Selection: FedNorm]{Highest global validation Dice scores for \fednorm with different interpolation ratios $\beta$ and varying numbers of
										modes $M$ per modality reported within 100 FL rounds of training. The best (overall highest) global validation Dice score in the table
										is highlighted in bold.}\label{tab:model-selection-fednorm}
	\centering
		\begin{tabular}{c c c c c}
			\toprule
			\multirow{2}{*}{\shortstack{\textbf{Interpolation}\\\textbf{Ratio} $\boldsymbol{(\beta)}$}}	& \multicolumn{4}{c}{\textbf{\# Modes} ($\boldsymbol{M}$)}	 			\\
																								& \textbf{1}	& \textbf{2}	& \textbf{3}		& \textbf{4}	\\
			\midrule
			1.0																					& 0.877			& 0.881			& 0.877				& 0.872			\\
			0.9																					& 0.883			& 0.881			& $\mathbf{0.893}$	& 0.881			\\
			0.5																					& 0.867			& 0.881			& 0.879				& 0.883			\\
			0.2																					& 0.833			& 0.805			& 0.878				& 0.880			\\
			\bottomrule
		\end{tabular}
\end{table}

==> tables/results_methods_center.tex <==
% !TeX root = ../main.tex
% Add the above to each chapter to make compiling the PDF easier in some editors.
\begin{table*}[ht]
	\caption[Comparison: Non-IID 3 Setting]{Comparison on the Non-IID 1 and 2 settings. The numbers give the performances of the local models, the centralized model, and the
											federated global models (without refinement at the clients) on the test set of each client. \fedavgm~\cite{FedAvgM} and \fednorm
											are not included for the Non-IID 2 setting because \fedavgm fails during training in this setting and \fednorm cannot handle
											mixed-modality clients. The performances are reported with Dice per patient and are given by mean (median) and standard deviation.
											Additionally, the RI~\cite{RelativeImprovement} is computed for the mean Dice per patient of the models from the FL algorithms and the centralized models over the local model
											performances. Hence, the RI is not reported for the local models. The best score from the federated models per setting and client is highlighted
											in bold. A star ($^\ast$) before/after the method name indicates that the results are statistically significant in the Non-IID 1/2 setting
											with a $p$-value $\leq 0.05$ using the unpaired two-sided t-test on the Dice per patient scores from the local model
											and the respective federated/centralized model.}\label{tab:comparison}
	\centering
	\begin{adjustbox}{max width=\textwidth, max height=0.45\textheight}
		\begin{tabular}{c c c c c c c}
 			\toprule
			\multicolumn{3}{c}{\textbf{Non-IID 1}} & \multirow{3.5}{*}{\textbf{Methods}} & \multicolumn{3}{c}{\textbf{Non-IID 2}}   \\
			\cmidrule{1-3} \cmidrule{5-7}
			\textbf{Client}	    & \textbf{Dice per}                         & \textbf{RI} $\boldsymbol{\uparrow}$   &   & \textbf{Dice per}                      
			& \textbf{RI} $\boldsymbol{\uparrow}$   & \textbf{Client}	    \\
			\textbf{(Modality)} & \textbf{Patient} $\boldsymbol{\uparrow}$	& \textbf{[\%]} 			            &   & \textbf{Patient} $\boldsymbol{\uparrow}$	
			& \textbf{[\%]}                         & \textbf{(Modality)}   \\
			\midrule
			\multirow{9}{*}{\shortstack{Multi-Atlas\\(CT)}}	& $0.850\,(0.862) \pm 0.050$  & -    & Local				& $0.850\,(0.862) \pm 0.050$	& -	& \multirow{9}{*}{\shortstack{Multi-Atlas\\(CT)}} 	\\
															\cdashline{2-6}
															& $0.883\,(0.899) \pm 0.071$  & 3.9 	& FedAvg$^\ast$~\cite{FedAvg}	& $0.906\,(0.907) \pm 0.042$	& 6.6	&  	\\
															& $0.575\,(0.541) \pm 0.150$  & -32.4 	& $^\ast$FedAvgM~\cite{FedAvgM}& -	                & -	&  	\\
															& $0.884\,(0.885) \pm 0.036$  & 4.0 	& $^\ast$FedVC~\cite{FedVC}	& $0.848\,(0.843) \pm 0.056$	& -0.2	&  	\\
															& $0.870\,(0.909) \pm 0.117$  & 2.4 	& SiloBN$^\ast$~\cite{SiloBN}	& $0.894\,(0.895) \pm 0.045$	& 5.2	&  	\\
															& $0.900\,(0.921) \pm 0.053$  & 5.9 	& $^\ast$FedBN$^\ast$~\cite{FedBN}	& $\boldsymbol{0.916\,(0.919) \pm 0.034}$	& \textbf{7.8}	&  	\\
															& $\boldsymbol{0.921\,(0.932) \pm 0.033}$  & \textbf{8.4} 	& $^\ast$FedNorm				& -                 & -	& 	\\
															& $0.891\,(0.898) \pm 0.034$  & 4.8 	& $^\ast$FedNorm+$^\ast$				& $\boldsymbol{0.916\,(0.928) \pm 0.030}$	& \textbf{7.8}	& 	\\
															\cdashline{2-6}
															& $0.921\,(0.934) \pm 0.033$  & 8.4 	& $^\ast$Centralized$^\ast$			& $0.894\,(0.914) \pm 0.061$	& 5.2	&  	\\
 			\midrule
 			\multirow{9}{*}{\shortstack{3D-IRCADb\\(CT)}}	& $0.918\,(0.926) \pm 0.029$  & -       & Local				& $0.918\,(0.926) \pm 0.029$	& -	& \multirow{9}{*}{\shortstack{3D-IRCADb\\(CT)}} 	\\
															\cdashline{2-6}
															& $0.940\,(0.942) \pm 0.018$  & 2.4 	& FedAvg~\cite{FedAvg}	& $0.933\,(0.946) \pm 0.037$	& 1.6	&  	\\
															& $0.874\,(0.888) \pm 0.036$  & -4.8 	& $^\ast$FedAvgM~\cite{FedAvgM}& -                 & -	&  	\\
															& $0.929\,(0.933) \pm 0.022$  & 1.2 	& FedVC~\cite{FedVC}	& $0.916\,(0.916) \pm 0.024$	& -0.2	&  	\\
															& $0.954\,(0.958) \pm 0.014$  & 3.9 	& $^\ast$SiloBN$^\ast$~\cite{SiloBN}	& $\boldsymbol{0.961\,(0.967) \pm 0.011}$	& \textbf{4.7}	&  	\\
															& $0.954\,(0.954) \pm 0.015$  & 3.9 	& $^\ast$FedBN$^\ast$~\cite{FedBN}	& $0.960\,(0.963) \pm 0.011$	& 4.6	&  	\\
															& $\boldsymbol{0.956\,(0.959) \pm 0.017}$  & \textbf{4.1} 	& $^\ast$FedNorm				& -                 & -	& 	\\
															& $0.942\,(0.942) \pm 0.016$  & 2.6 	& FedNorm+$^\ast$				& $0.955\,(0.956) \pm 0.016$	& 4.0	& 	\\
															\cdashline{2-6}
															& $0.953\,(0.957) \pm 0.012$  & 3.8 	& $^\ast$Centralized			& $0.938\,(0.945) \pm 0.028$	& 2.2	&  	\\
 			\midrule
 			\multirow{9}{*}{\shortstack{SLIVER07\\(CT)}}	& $0.888\,(0.887) \pm 0.062$  & -    & Local				& $0.718\,(0.784) \pm 0.209$	& -	& \multirow{9}{*}{\shortstack{CHAOS19 MR\\T1 Water\\(MRI)}} 	\\
															\cdashline{2-6}
															& $0.888\,(0.924) \pm 0.135$  & 0.0 	& FedAvg~\cite{FedAvg}	& $0.421\,(0.472) \pm 0.339$	& -41.4	&  	\\
															& $0.761\,(0.785) \pm 0.122$  & -14.3 	& $^\ast$FedAvgM~\cite{FedAvgM}& -                 & -	&  	\\
															& $0.905\,(0.926) \pm 0.079$  & 1.9 	& FedVC$^\ast$~\cite{FedVC}	& $0.424\,(0.493) \pm 0.277$	& -40.9	&  	\\
															& $\boldsymbol{0.924\,(0.944) \pm 0.070}$  & \textbf{4.1} 	& SiloBN~\cite{SiloBN}	& $0.514\,(0.498) \pm 0.233$	& -28.4	&  	\\
															& $0.906\,(0.928) \pm 0.064$  & 2.0 	& FedBN~\cite{FedBN}	& $0.459\,(0.512) \pm 0.319$	& -36.1	&  	\\
															& $0.914\,(0.940) \pm 0.084$  & 2.9 	& FedNorm				& -                 & -	& 	\\
															& $0.883\,(0.903) \pm 0.116$  & -0.6 	& FedNorm+				& $\boldsymbol{0.759\,(0.754) \pm 0.065}$	& \textbf{5.7}	& 	\\
															\cdashline{2-6}
															& $0.934\,(0.943) \pm 0.057$  & 5.2 	& Centralized			& $0.893\,(0.879) \pm 0.082$	& 24.4	&  	\\
			\midrule
			\multirow{9}{*}{\shortstack{CHAOS19 MR\\T1 In-Phase\\(MRI)}}	& $0.254\,(0.278) \pm 0.168$  & -   & Local & $0.865\,(0.870) \pm 0.043$	& -	& \multirow{9}{*}{\shortstack{KORA\\T1 Water (1)\\(MRI)}} 	\\
															\cdashline{2-6}
															& $0.460\,(0.511) \pm 0.233$  & 81.1 	& FedAvg$^\ast$~\cite{FedAvg}	& $0.930\,(0.935) \pm 0.030$	& 7.5	&  	\\
															& $0.579\,(0.661) \pm 0.199$  & 128.0 	& $^\ast$FedAvgM~\cite{FedAvgM}& -                 & -	&  	\\
															& $0.228\,(0.070) \pm 0.301$  & -10.2 	& FedVC~\cite{FedVC}	& $0.893\,(0.896) \pm 0.044$	& 3.2	&  	\\
															& $0.656\,(0.678) \pm 0.185$  & 158.3 	& $^\ast$SiloBN$^\ast$~\cite{SiloBN}	& $0.932\,(0.933) \pm 0.026$	& 7.7	&  	\\
															& $0.386\,(0.485) \pm 0.333$  & 52.0 	& FedBN$^\ast$~\cite{FedBN}	& $\boldsymbol{0.941\,(0.945) \pm 0.021}$	& \textbf{8.8}	&  	\\
															& $\boldsymbol{0.795\,(0.851) \pm 0.170}$  & \textbf{213.0} 	& $^\ast$FedNorm				& -                 & -	& 	\\
															& $0.653\,(0.803) \pm 0.303$  & 157.1 	& $^\ast$FedNorm+$^\ast$				& $0.938\,(0.941) \pm 0.022$	& 8.4	& 	\\
															\cdashline{2-6}
															& $0.688\,(0.869) \pm 0.369$  & 170.9 	& $^\ast$Centralized$^\ast$			& $0.936\,(0.939) \pm 0.024$	& 8.2	&  	\\
			\midrule
            \multirow{9}{*}{\shortstack{CHAOS19 MR\\T1 Out-Phase\\(MRI)}}	& $0.704\,(0.735) \pm 0.182$  & -   & Local & $0.703\,(0.872) \pm 0.348$	& -	& \multirow{9}{*}{\shortstack{SLIVER07\\+ KORA T1\\Water (2)\\(CT + MRI)}} 	\\
															\cdashline{2-6}
															& $0.443\,(0.477) \pm 0.237$  & -37.1 	& $^\ast$FedAvg~\cite{FedAvg}	& $0.793\,(0.928) \pm 0.282$	& 12.8	&  	\\
															& $0.590\,(0.672) \pm 0.248$  & -16.2 	& FedAvgM~\cite{FedAvgM}& -                 & -	&  	\\
															& $0.296\,(0.285) \pm 0.307$  & -58.0 	& $^\ast$FedVC~\cite{FedVC}	& $0.733\,(0.886) \pm 0.333$	& 4.3	&  	\\
															& $0.735\,(0.713) \pm 0.137$  & 4.4 	& SiloBN~\cite{SiloBN}	& $\boldsymbol{0.823\,(0.923) \pm 0.214}$	& \textbf{17.1}	&  	\\
															& $0.444\,(0.460) \pm 0.358$  & -36.9 	& FedBN~\cite{FedBN}	& $0.784\,(0.927) \pm 0.282$	& 11.5	&  	\\
															& $\boldsymbol{0.777\,(0.786) \pm 0.090}$  & \textbf{10.4} 	& FedNorm				& -                 & -	& 	\\
															& $0.661\,(0.752) \pm 0.271$  & -6.1 	& FedNorm+				& $0.755\,(0.933) \pm 0.347$	& 7.4	& 	\\
															\cdashline{2-6}
															& $0.716\,(0.867) \pm 0.318$  & 1.7 	& Centralized			& $0.844\,(0.925) \pm 0.165$	& 20.1	&  	\\
            \midrule
            \multirow{9}{*}{\shortstack{CHAOS19 MR\\T1 Water\\(MRI)}}	& $0.718\,(0.784) \pm 0.209$  & -    & Local	& $0.885\,(0.918) \pm 0.089$	& -	& \multirow{9}{*}{\shortstack{LiTS17\\Site 2\\+ KORA T1\\Water (3)\\(CT + MRI)}} 	\\
															\cdashline{2-6}
															& $0.481\,(0.578) \pm 0.280$  & -33.0 	& FedAvg~\cite{FedAvg}	& $0.932\,(0.953) \pm 0.050$	& 5.3	&  	\\
															& $0.604\,(0.672) \pm 0.240$  & -15.9 	& FedAvgM~\cite{FedAvgM}& -                 & -	&  	\\
															& $0.291\,(0.248) \pm 0.311$  & -59.5 	& $^\ast$FedVC~\cite{FedVC}	& $0.882\,(0.909) \pm 0.089$	& -0.3	&  	\\
															& $0.683\,(0.685) \pm 0.164$  & -4.9 	& SiloBN~\cite{SiloBN}	& $0.918\,(0.942) \pm 0.070$	& 3.7	&  	\\
															& $0.467\,(0.543) \pm 0.342$  & -35.0 	& FedBN~\cite{FedBN}	& $0.810\,(0.915) \pm 0.174$	& -8.5	&  	\\
															& $\boldsymbol{0.807\,(0.841) \pm 0.126}$  & \textbf{12.4} 	& FedNorm				& -                 & -	& 	\\
															& $0.680\,(0.784) \pm 0.285$  & -5.3 	& FedNorm+$^\ast$				& $\boldsymbol{0.942\,(0.946) \pm 0.023}$	& \textbf{6.4}	& 	\\
															\cdashline{2-6}
															& $0.744\,(0.893) \pm 0.317$  & 3.6 	& Centralized			& $0.938\,(0.950) \pm 0.035$	& 6.0	&  	\\
 			\bottomrule
		\end{tabular}
	\end{adjustbox}
\end{table*}
